Optimal control problems with free right end point

This paper is dedicated to the elementary proof of Pontryagin's maximum principle for problems with free right end point. The proof for the standard problem is taken from the monography of Ioffe and Tichomirov. We assume piecewise continuous controls and the proof turns out to be very simple. We generalize the concept to the problem of optimal multiprocesses, to control problems with delays and to the control of Volterra integral equations. Furthermore, we discuss the problem on infinite horizon. Moreover, we state Arrow type sufficiency conditions. The optimality conditions are demonstrated on illustrative examples.

==> 4-1-Vorbereitungen.tex <==
\subsection{Vorbereitende Betrachtungen} \label{AbschnittVorbereitungenRet}
Bei der Behandlung von Steuerungsproblemen mit einer Zeitverzögerung stellt sich die Frage,
wie über dem Zeitintervall $[a,b]$ das dynamische System
$$\dot{x}(t) = \varphi\big(t,x(t),x(t-\Delta)\big), \quad x(t)=x_a \mbox{ für } t \in [a-\Delta,a],$$
zu behandeln ist.
Für den Teilabschnitt $[a,a+\Delta]$ reduziert es sich auf die Gleichung
$$\dot{x}(t) = \varphi\big(t,x(t),x_a\big), \quad x(a)=x_a,$$
welche sich für eine stückweise stetige rechte Seite $\varphi$ mit den Werkzeugen im Anhang \ref{AnhangDGL} über Differentialgleichungen handhaben lässt.
Dieser Gedankengang kann anschließend schrittweise über den Teilabschnitten $[a+\Delta,a+2\Delta]$, $[a+2\Delta,a+3\Delta]$, ... wiederholt werden.
Auf die gleiche Weise ergibt sich über $[a,b]$ die Lösung der Gleichung
$$\dot{y}(t) = \psi\big(t,y(t),y(t+\Delta)\big), \quad y(t)=y_b \mbox{ für } t \in [b,b+\Delta],$$
in umgekehrter Zeitrichtung,
indem man zunächst die Gleichung
$$\dot{y}(t) = \psi\big(t,y(t),y_b\big), \quad y(b)=y_b,$$
über $[b-\Delta,b]$ und dann sukzessive über $[b-2\Delta,b-\Delta]$, $[b-3\Delta,b-2\Delta]$, ... löst.
Daher kann die Dynamik mit Zeitverzögerung stückweise wie eine Differentialgleichung mit stückweise stetigen rechten Seiten
aufgefasst werden. \\[2mm]
Im Zuge des Beweises gelangen wir zu Ausdrücken, welche Verzögerungen in verschiedene Zeitrichtungen aufweisen.
Mit der Substitution $t = s+ \Delta$ gilt $f(t)g(t-\Delta)=f(s+\Delta)g(s)$ und es ergibt sich (nach Umbenennung von $s$ zu $t$) die Beziehung
%$$f(t)g(t-\Delta)=f(s+\Delta)g(s) \quad \mbox{ mit } t \in [a+\Delta,b],\, t \in [a,b-\Delta].$$
%Damit ergibt sich die Beziehung
\begin{equation}\label{Zeitshift}
\int_a^b \chi_{[c+\Delta,d]}(t) \cdot f(t)g(t-\Delta) \, dt = \int_a^b \chi_{[c,d-\Delta]}(t) \cdot f(t+\Delta)g(t) \, dt.
\end{equation}

==> 5-5-Interpretation.tex <==
\subsection{\"Okonomische Deutung des Maximumprinzips} \label{AbschnittInterpretationIGL}
\index{Pontrjaginsches Maximumprinzip!oekonomische@--, ökonomische Interpretation}
Bevor wir uns der Interpretation in Abschnitt \ref{AbschnittDeutung} anschließen,
geben wir eine ``unverfälschte'' Variante von Theorem \ref{SatzPMPeinfachIGL} an.
Die Umformulierung basiert auf der Beziehung (\ref{StieltjesIGL}) für das Stieltjes-Integral.
Der Akzent von (\ref{StieltjesIGL}) beruht in der Unstetigkeitsstelle der Funktion $g(\cdot)$ im Endpunkt,
welche zur Sprungbedingung auf der rechten Seite führt. \\[2mm]
Da in der Pontrjagin-Funktion $H_0^{\mathcal{I}}(t,x,u,p(\cdot))$ durch den Term $\langle \varphi(t_1,t,x,u), p(t_1)\rangle$
die Sprungbedingung bereits Beachtung gefunden hat,
wurde in Theorem \ref{SatzPMPeinfachIGL} die Adjungierte $p(\cdot)$ stückweise stetig diferenzierbar auf $[t_0,t_1]$ fortgesetzt,
dem Raum $PC_1([t_0,t_1],\R^n)$ zugeordnet und die Transversalitätsbedingung $p(t_1)=-S'\big(x_*(t_1)\big)$ formuliert. \\
Führt man die Sprungbedingung wiederum zurück auf die linke Seite der Beziehung (\ref{StieltjesIGL}),
so ergibt sich die Pontrjagin-Funktion ohne Randterm, 
$$H^{\mathcal{I}}(t,x,u,q(\cdot)\big) = -\int_t^{t_1} \langle \varphi(\tau,t,x,u), dq(\tau) \rangle - f(t,x,u),$$
und die Funktion $q(\cdot) \in PC_1([t_0,t_1),\R^n)$ mit $q(t_1^-)=p(t_1)$ und $q(t_1)=0$.
Ferner erhält man eine Version des Maximumprinzips mit Sprung-Transversalitätsbedingung:

\begin{theorem}[Pontrjaginsches Maximumprinzip] \label{SatzPMPeinfachIGL2}
\index{Pontrjaginsches Maximumprinzip!Integral@-- Integralgleichungen} 
Sei $\big(x_*(\cdot),u_*(\cdot)\big) \in \mathscr{A}^{\mathcal{I}}_{\rm adm} \cap \mathscr{A}^{\mathcal{I}}_{\rm Lip}$. 
Ist $\big(x_*(\cdot),u_*(\cdot)\big)$ ein starkes lokales Minimum der Aufgabe (\ref{PMPeinfachIGL1})--(\ref{PMPeinfachIGL3}),
dann existiert eine Vektorfunktion $q(\cdot) \in PC_1([t_0,t_1),\R^n)$ derart, dass
\begin{enumerate}
\item[(a)] die adjungierte Gleichung
           \index{adjungierte Gleichung!Integral@-- Integralgleichungen}
           \begin{equation} \label{SatzPMPIGL1}
           \dot{q}(t) = \int_t^{t_1} \langle \varphi_x\big(\tau,t,x_*(t),u_*(t)\big), dq(\tau) \rangle + f_x\big(t,x_*(t),u_*(t)\big),
           \end{equation}
\item[(b)] in $t=t_1$ die Sprung-Transversalitätsbedingung
           \index{Transversalitätsbedingungen!Integral@-- Integralgleichungen}
           \begin{equation} \label{SatzPMPIGL2} q(t_1^-)=-S'\big(x_*(t_1)\big), \qquad q(t_1)=0, \end{equation}
\item[(c)] in fast allen Punkten $t \in [t_0,t_1]$ die Maximumbedingung
           \index{Maximumbedingung!Integral@-- Integralgleichungen}
           \begin{equation} \label{SatzPMPIGL3}
           H^{\mathcal{I}}\big(t,x_*(t),u_*(t),q(\cdot)\big) = \max_{u \in U} \tilde{H}^{\mathcal{I}}\big(t,x_*(t),u,q(\cdot)\big).
           \end{equation}
\end{enumerate}
erfüllt sind.
\end{theorem}

In Verallgemeinerung zu Abschnitt \ref{AbschnittDeutung},
wo $v \to H^{\mathcal{S}}\big(\tau,x_*(\tau),v,p(\tau)\big)$ die Profitrate aus direktem $f\big(\tau,x_*(\tau),v\big)$
und indirektem Gewinn $\big\langle p(\tau) , \varphi\big(\tau,x_*(\tau),v\big) \big\rangle$ bemisst,
enthält $H^{\mathcal{I}}$ den Erwartungswert
$\displaystyle \int_\tau^{t_1} \big\langle \varphi\big(t,\tau,x_*(\tau),v\big), dq(t) \big\rangle$
zum Gewicht $q(\cdot)$ über die gesamte künftige Entwicklung des indirekten Gewinnes.


==> 5-8-Fredholm.tex <==
\subsection{Die Fredholmsche Integralgleichung}
Unsere Ausführungen zur Aufgabe (\ref{PMPeinfachIGL1})--(\ref{PMPeinfachIGL3}) versetzen uns unmittelbar in die Lage
die Steuerung einer Fredholmschen Integralgleichung,
d.\,h. die Aufgabe 
\begin{eqnarray}
&&\label{PMPeinfachIGLF1} J\big(x(\cdot),u(\cdot)\big) = \int_{t_0}^{t_1} f\big(t,x(t),u(t)\big) \, dt  +S\big(x(t_1)\big) \to \inf, \\
&&\label{PMPeinfachIGLF2} x(t) = x_0 + \int_{t_0}^{t_1} \varphi\big(t,s,x(s),u(s)\big) \, ds, \quad t \in [t_0,t_1], \\
&&\label{PMPeinfachIGLF3} u(t) \in U \subseteq \R^m, \quad U \not= \emptyset
\end{eqnarray}
bez"uglich $\big(x(\cdot),u(\cdot)\big) \in PC_1([t_0,t_1],\R^n) \times PC([t_0,t_1],U)$ zu untersuchen. \\[2mm]
Wir übernehmen an dieser Stelle die Voraussetzungen und Bezeichnungen aus Abschnitt \ref{AbschnittPMPeinfachIGL}.
Ferner bezeichnen 
\begin{eqnarray*}
H^{\mathcal{F}}(t,x,u,p(\cdot)\big) &=& -\int_{t_0}^{t_1} \langle \varphi(\tau,t,x,u), dp(\tau) \rangle - f(t,x,u), \\
H_0^{\mathcal{F}}(t,x,u,p(\cdot)\big) &=& -\int_{t_0}^{t_1} \langle \varphi(\tau,t,x,u), \dot{p}(\tau) \rangle \, d\tau
                                    +\langle \varphi(t_1,t,x,u), p(t_1)\rangle - f(t,x,u)
\end{eqnarray*}
die Pontrjagin-Funktionen der Aufgabe (\ref{PMPeinfachIGLF1})--(\ref{PMPeinfachIGLF3}).

\begin{theorem}[Pontrjaginsches Maximumprinzip] \label{SatzPMPeinfachIGLF2}
\index{Pontrjaginsches Maximumprinzip!Integral@-- Integralgleichungen} 
Sei $\big(x_*(\cdot),u_*(\cdot)\big) \in \mathscr{A}^{\mathcal{I}}_{\rm adm} \cap \mathscr{A}^{\mathcal{I}}_{\rm Lip}$. 
Ist $\big(x_*(\cdot),u_*(\cdot)\big)$ ein starkes lokales Minimum der Aufgabe (\ref{PMPeinfachIGLF1})--(\ref{PMPeinfachIGLF3}),
dann existiert eine Vektorfunktion $p(\cdot) \in PC_1([t_0,t_1),\R^n)$ derart, dass
\begin{enumerate}
\item[(a)] die adjungierte Gleichung
           \index{adjungierte Gleichung!Integral@-- Integralgleichungen}
           \begin{eqnarray} 
           \dot{p}(t) &=& -H_x^{\mathcal{F}}\big(t,x_*(t),u_*(t),p(\cdot)\big) \nonumber \\
                      &=& \label{SatzPMPIGLF1} \int_{t_0}^{t_1} \varphi^T_x\big(\tau,t,x_*(t),u_*(t)\big)\, dp(\tau) + f_x\big(t,x_*(t),u_*(t)\big),
           \end{eqnarray}
\item[(b)] in $t=t_1$ die Sprung-Transversalitätsbedingung
           \index{Transversalitätsbedingungen!Integral@-- Integralgleichungen}
           \begin{equation} \label{SatzPMPIGLF2} p(t_1^-)=-S'\big(x_*(t_1)\big), \qquad p(t_1)=0, \end{equation}
\item[(c)] in fast allen Punkten $t \in [t_0,t_1]$ die Maximumbedingung
           \index{Maximumbedingung!Integral@-- Integralgleichungen}
           \begin{equation} \label{SatzPMPIGLF3}
           H^{\mathcal{F}}\big(t,x_*(t),u_*(t),p(\cdot)\big) = \max_{u \in U} H^{\mathcal{F}}\big(t,x_*(t),u,p(\cdot)\big).
           \end{equation}
\end{enumerate}
erfüllt sind.
\end{theorem}

Beachten wir den Zusammenhang zwischen den Pontrjagin-Funktionen $H^{\mathcal{F}}(t,x,u,p(\cdot)\big)$ und $H_0^{\mathcal{F}}(t,x,u,p(\cdot)\big)$
mittels der Sprungbedingung von der Adjungierten $p(\cdot)$ in $t=t_1$,
so erhalten wir unmittelbar die folgende Form von Theorem \ref{SatzPMPeinfachIGLF2}:
  
\begin{theorem}[Pontrjaginsches Maximumprinzip] \label{SatzPMPeinfachIGLF}
\index{Pontrjaginsches Maximumprinzip!Integral@-- Integralgleichungen} 
Sei $\big(x_*(\cdot),u_*(\cdot)\big) \in \mathscr{A}^{\mathcal{I}}_{\rm adm} \cap \mathscr{A}^{\mathcal{I}}_{\rm Lip}$. 
Ist $\big(x_*(\cdot),u_*(\cdot)\big)$ ein starkes lokales Minimum der Aufgabe (\ref{PMPeinfachIGL1})--(\ref{PMPeinfachIGL3}),
dann existiert eine Vektorfunktion $p(\cdot) \in PC_1([t_0,t_1],\R^n)$ derart, dass
\begin{enumerate}
\item[(a)] die adjungierte Gleichung
           \index{adjungierte Gleichung!Integral@-- Integralgleichungen}
           \begin{equation}\label{PMPeinfachIGLF4} 
           \dot{p}(t) = -H_{0x}^{\mathcal{F}}\big(t,x_*(t),u_*(t),p(\cdot)\big),
           \end{equation}
\item[(b)] in $t=t_1$ die Transversalitätsbedingung
           \index{Transversalitätsbedingungen!Integral@-- Integralgleichungen}
           \begin{equation}\label{PMPeinfachIGLF5} p(t_1)=-S'\big(x_*(t_1)\big), \end{equation}
\item[(c)] in fast allen Punkten $t \in [t_0,t_1]$ die Maximumbedingung
           \index{Maximumbedingung!Integral@-- Integralgleichungen}
           \begin{equation}\label{PMPeinfachIGLF6} 
           H_0^{\mathcal{F}}\big(t,x_*(t),u_*(t),p(\cdot)\big) = \max_{u \in U} H_0^{\mathcal{F}}\big(t,x_*(t),u,p(\cdot)\big).
           \end{equation}
\end{enumerate}
erfüllt sind.
\end{theorem}

{\bf Beweis} Wir übernehmen die Bezeichnungen aus Abschnitt \ref{AbschnittPMPBeweiseinfachIGL} und erhalten wie ebenda:
Für $t \in [t_0,t_1]$ ergibt sich
\begin{eqnarray*}
x_{\lambda}(t) - x_*(t)
&=& \int_{t_0}^{t_1} \big[ \varphi\big(t,s,x_\lambda(s),u_\lambda(s)\big) - \varphi\big(t,s,x_*(s),u_*(s)\big) \big] \, ds \\
&=& \int_{t_0}^{t_1} \big[ \varphi\big(t,s,x_\lambda(s),u_*(s)\big) - \varphi\big(t,s,x_*(s),u_*(s)\big) \big] \, ds \\
& & + \int_{\tau-\lambda}^{\tau} \big[ \varphi\big(t,s,x_\lambda(s),u_\lambda(s)\big) - \varphi\big(t,s,x_\lambda(s),u_*(s)\big) \big] \, ds.
\end{eqnarray*}
Wegen der gleichmäßigen Konvergenz von $x_\lambda(\cdot)$ gegen $x_*(\cdot)$ für $\lambda \to 0^+$
liefert dieser Grenzübergang für $\displaystyle y(t)=\lim_{\lambda \to 0^+}\frac{x_{\lambda}(t) - x_*(t)}{\lambda}$
die Darstellung
\begin{eqnarray}
y(t) &=&  \underbrace{\varphi\big(t,\tau,x_*(\tau),v\big) - \varphi\big(t,\tau,x_*(\tau),u_*(\tau)\big)}_{=y(\tau;t)}
          + \int_{t_0}^{t_1} \varphi_x[t,s] y(s) \, ds \nonumber \\
     &=& \label{BeweisPMPeinfachIGLF1} y(\tau;t) + \int_{t_0}^{t_1} \varphi_x[t,s]\,y(s) \, ds.
\end{eqnarray} 
Mit der adjungierten Gleichung (\ref{PMPeinfachIGLF4}) erhalten wir:
\begin{eqnarray}
  \int_{t_0}^{t_1} \langle f_x[t] , y(t) \rangle \, dt
&=& \int_{t_0}^{t_1} \langle \dot{p}(t) , y(t) \rangle \, dt 
    - \int_{t_0}^{t_1} \Big\langle \int_{t_0}^{t_1} \varphi^T_x[s,t] \dot{p}(s) \, ds, y(t) \Big\rangle \, dt\nonumber \\
&& \label{BeweisPMPeinfachIGLF2} + \int_{t_0}^{t_1} \langle \varphi^T_x[t_1,t] p(t_1^-) , y(t) \rangle \, dt.
\end{eqnarray}
Für die beiden ersten Terme in (\ref{BeweisPMPeinfachIGLF2}) führt (\ref{BeweisPMPeinfachIGLF1}) unmittelbar zu dem Zusammenhang
$$\int_{t_0}^{t_1} \langle \dot{p}(t) , y(t) \rangle \, dt 
    - \int_{t_0}^{t_1} \Big\langle \int_{t_0}^{t_1} \varphi^T_x[s,t] \dot{p}(s) \, ds, y(t) \Big\rangle \, dt
   = \int_{t_0}^{t_1} \langle \dot{p}(t) , y(\tau;t) \rangle \, dt.$$
In der Gleichung (\ref{BeweisPMPeinfachIGLF1}) gilt $\displaystyle y(t_1)-y(\tau;t_1) = \int_{t_0}^{t_1} \varphi_x\big[t_1,t] y(t) \, dt$
für $t=t_1$ und es folgt für den dritten Term in (\ref{BeweisPMPeinfachIGLF2}) die Beziehung
$$\int_{t_0}^{t_1} \langle p(t_1^-) , \varphi_x[t_1,t]y(t) \rangle \, dt
  = \Big\langle p(t_1^-), \int_{t_0}^{t_1} \varphi_x[t_1,t]y(t) \, dt \Big\rangle = \langle p(t_1^-) ,y(t_1)-y(\tau;t_1) \rangle.$$
Beachten wir nun die Transversalitätsbedingung $p(t_1^-)=-S'\big(x_*(t_1)\big)$, so ergibt sich
\begin{equation} \label{BeweisPMPeinfachIGLF3}
\int_{t_0}^{t_1} \langle f_x[t] , y(t) \rangle \, dt + \langle S'\big(x_*(t_1)\big) ,y(t_1) \rangle
   = \int_{t_0}^{t_1} \langle \dot{p}(t) , y(\tau;t) \rangle \, dt - \langle p(t_1^-) ,y(\tau;t_1) \rangle.
\end{equation}
Da $\big(x_*(\cdot),u_*(\cdot)\big)$ ein starkes lokales Minimum ist, gilt
\begin{eqnarray*}
0 &\leq& \lim_{\lambda \to 0^+} \frac{J\big(x_\lambda(\cdot),u_\lambda(\cdot)\big)- J\big(x_*(\cdot),u_*(\cdot)\big)}{\lambda} \\
  &=   & f\big(\tau,x_*(\tau),v\big) - f\big(\tau,x_*(\tau),u_*(\tau)\big)
         + \int_{t_0}^{t_1} \big\langle f_x[t],y(t) \big\rangle \, dt + \langle S'\big(x_*(t_1)\big) ,y(t_1) \rangle.
\end{eqnarray*}
Mit (\ref{BeweisPMPeinfachIGLF3}) und der Setzung von $y(\tau;t)$ in (\ref{BeweisPMPeinfachIGLF1}) ergibt sich hieraus die Ungleichung
$$0 \leq f\big(\tau,x_*(\tau),v\big) - f\big(\tau,x_*(\tau),u_*(\tau)\big)
         + \int_{t_0}^{t_1} \langle \dot{p}(t) , y(\tau;t) \rangle \, dt - \langle p(t_1^-) ,y(\tau;t_1) \rangle,$$
die äquivalent zu der Ungleichung
$$H^{\mathcal{F}}\big(\tau,x_*(\tau),v,p(\cdot)\big) \leq H^{\mathcal{F}}\big(\tau,x_*(\tau),u_*(\tau),p(\cdot)\big)$$
ist.
Da $\tau$ ein beliebiger Stetigkeitspunkt von $u_*(\cdot)$ und $v$ ein beliebiger Punkt der Menge $U$ war,
zeigt diese Ungleichung die Gültigkeit der Maximumbedingung (\ref{PMPeinfachIGLF6}). \hfill $\blacksquare$ \\[2mm]
Wir gehen nun auf hinreichende Bedingungen nach Arrow\index{hinreichende Bedingungen nach Arrow!Integral@-- Integralgleichungen}
für die Aufgabe (\ref{PMPeinfachIGLF1})--(\ref{PMPeinfachIGLF3}) ein.
Dabei geben wir wieder zwei Varianten an, die sich auf die Darstellungen der Optimalitätsbedingungen der Theoreme
\ref{SatzPMPeinfachIGLF2} und \ref{SatzPMPeinfachIGLF} beziehen.
Für $t \in [t_0,t_1]$ bezeichnet $V^{\mathcal{I}}_\gamma(t)$ im Folgenden erneut die Menge
$$V^{\mathcal{I}}_\gamma(t)=\{ x \in \R^n \,|\, \|x-x_*(t)\| \leq \gamma\}.$$
Die erste Variante der hinreichenden Bedingungen bezieht sich auf Theorem \ref{SatzPMPeinfachIGLF2}.
Hier lautet die zugehörige ``unverfälschte'' Hamilton-Funktion
$$\mathscr{H}^{\mathcal{F}}\big(t,x,p(\cdot)\big)
  = \sup_{u \in U} \bigg[-\int_{t_0}^{t_1} \langle \varphi(\tau,t,x,u), dp(\tau) \rangle - f(t,x,u)\bigg].$$

\begin{theorem} \label{SatzHBPMPIGF2}
In der Aufgabe (\ref{PMPeinfachIGLF1})--(\ref{PMPeinfachIGLF3}) sei
$\big(x_*(\cdot),u_*(\cdot)\big) \in \mathscr{A}^{\mathcal{I}}_{\rm adm} \cap \mathscr{A}^{\mathcal{I}}_{\rm Lip}$
und es sei $p(\cdot) \in PC_1([t_0,t_1),\R^n)$. Ferner gelte:
\begin{enumerate}
\item[(a)] Das Tripel $\big(x_*(\cdot),u_*(\cdot),p(\cdot)\big)$
           erf"ullt (\ref{SatzPMPIGLF1})--(\ref{SatzPMPIGLF3}) in Theorem \ref{SatzPMPeinfachIGLF2}.        
\item[(b)] F"ur jedes $t \in [t_0,t_1]$ ist die Funktion $\mathscr{H}^{\mathcal{F}}\big(t,x,p(t)\big)$ konkav in $x$ auf $V^{\mathcal{I}}_\gamma(t)$.
\item[(c)] Die Abbildung $S:\R^n\to \R$ im Zielfunktional (\ref{PMPeinfachIGLF1}) ist konvex in $x$ auf $V^{\mathcal{I}}_\gamma(t_1)$.
\end{enumerate}
Dann ist $\big(x_*(\cdot),u_*(\cdot)\big)$ ein starkes lokales Minimum der Aufgabe (\ref{PMPeinfachIGLF1})--(\ref{PMPeinfachIGLF3}).
\end{theorem}

Die zweite Variante der hinreichenden Bedingungen beruht auf Theorem \ref{SatzPMPeinfachIGLF}.
In diesem Fall hat die Hamilton-Funktion die Gestalt
$$\mathscr{H}_0^{\mathcal{F}}\big(t,x,p(\cdot)\big)
  = \sup_{u \in U} \bigg[-\int_{t_0}^{t_1} \langle \varphi(\tau,t,x,u), \dot{p}(\tau) \rangle \, d\tau
                                    +\langle \varphi(t_1,t,x,u), p(t_1)\rangle - f(t,x,u)\bigg].$$

\begin{theorem} \label{SatzHBPMPIGF1}
In der Aufgabe (\ref{PMPeinfachIGLF1})--(\ref{PMPeinfachIGLF3}) sei
$\big(x_*(\cdot),u_*(\cdot)\big) \in \mathscr{A}^{\mathcal{I}}_{\rm adm} \cap \mathscr{A}^{\mathcal{I}}_{\rm Lip}$
und es sei $p(\cdot) \in PC_1([t_0,t_1],\R^n)$. Ferner gelte:
\begin{enumerate}
\item[(a)] Das Tripel $\big(x_*(\cdot),u_*(\cdot),p(\cdot)\big)$
           erf"ullt (\ref{PMPeinfachIGLF4})--(\ref{PMPeinfachIGLF6}) in Theorem \ref{SatzPMPeinfachIGLF}.        
\item[(b)] F"ur jedes $t \in [t_0,t_1]$ ist die Funktion $\mathscr{H}_0^{\mathcal{F}}\big(t,x,p(t)\big)$ konkav in $x$ auf $V^{\mathcal{I}}_\gamma(t)$.
\item[(c)] Die Abbildung $S:\R^n\to \R$ im Zielfunktional (\ref{PMPeinfachIGL1}) ist konvex in $x$ auf $V^{\mathcal{I}}_\gamma(t_1)$.
\end{enumerate}
Dann ist $\big(x_*(\cdot),u_*(\cdot)\big)$ ein starkes lokales Minimum der Aufgabe (\ref{PMPeinfachIGLF1})--(\ref{PMPeinfachIGLF3}).
\end{theorem}

Die Beweise der Arrow-Bedingungen erfolgen auf die gleiche Weise wie im Abschnitt \ref{AbschnittArrowIGL}.
